DarkDiff: Explainable web page similarity of TOR onion sites

In large-scale data analysis, near-duplicates are often a problem. For example, with two near-duplicate phishing emails, a difference in the salutation (Mr versus Ms) is not essential, but whether it is bank A or B is important. The state-of-the-art in near-duplicate detection is a black box approach (MinHash), so one only knows that emails are near-duplicates, but not why. We present DarkDiff, which can efficiently detect near-duplicates while providing the reason why there is a near-duplicate. We have developed DarkDiff to detect near-duplicates of homepages on the Darkweb. DarkDiff works well on those pages because they resemble the clear web of the past.

==> tables_v5/tab_annotations.tex <==
% updated 20230315
% http://172.16.22.172/Domain_name/Result_10/Diff_word_all_loop_10_boilerplate/r_annotated_context_stat.html

\begin{table}
\caption{The top annotations of deletes and inserts with examples (10\% sample; N = 23,478,389)}
\label{tab:annotations}
\begin{tabular}{lrrr}
\toprule
Annotation	& \%	& Examples \\
\midrule
Bitcoin		&47.7	&https://www.blockchain.com/btc/address/ \\
\multicolumn{3}{r}{{\color{orange}3Lc18ENW1hWDHbZSrnws8mJt4zocpSAmFH}}\\
Price		&27.7	&{\color{red}0.00173}{\color{green}0.00174} BTC\\
Date		&14.5	&{\color{red}12/May}{\color{green}13/May}/2022\\
{\bf fail}	& 5.8	&wpnonce={\color{red}6d607}{\color{green}d08b4}\\
{\bf empty}	& 2.0	&\\
Ad		& 1.1	&{\color{red}17113}{\color{green}17132} Completed Orders\\
Space		& 0.3	& \\
Onion		& 0.3	&http://{\color{orange}facebookcorewwwi}.onion\\
Time		& 0.2	&{\color{red}8 days}{\color{green}2 weeks}\\
Image		& 0.1	&{\color{red}1-2}{\color{green}2-23}.png\\
\bottomrule
\end{tabular}
\end{table}


==> tables_v5/tab_no_alignment.tex <==
\begin{table*}
\caption{Computing the annotated templates for three versions without alignment}
\label{tab:no_alignment}
\begin{tabular}{lrlrll}
\toprule
	&Page version			&	&Diff					&	&Annotated template \\
\midrule
v1	&Lorem 2022-04-05 ipsum 1.0 BTC	&	&			$\nearrow$	&t1	&Lorem {\color{blue}date} ipsum 1.0 BTC \\
	&		$\searrow$	&d1\_2	&Lorem {\color{red}2022-04-05}		&	& \\
	&		$\nearrow$	&	&{\color{green}2022-04-06} ipsum 1.0 BTC&	& \\
v2	&Lorem 2022-04-06 ipsum 1.0 BTC	&	&			$\searrow$	&t2	&Lorem {\color{blue}date} ipsum 1.0 BTC \\
	&				&	&			$\nearrow$	&$\neq$t2'
												&Lorem 2022-04-06 ipsum {\color{blue}price } BTC \\
	&		$\searrow$	&d2\_3	&Lorem 2022-04-06			&	& \\
	&		$\nearrow$	&	&ipsum {\color{red}1.0} {\color{green}1.5} BTC
											&	& \\
v3	&Lorem 2022-04-06 ipsum 1.5 BTC	&	&			$\searrow$	&t3	&Lorem 2022-04-06 ipsum {\color{blue}price} BTC \\
\bottomrule
\end{tabular}
\end{table*}


==> tables_v5/tab_perfect_alignment.tex <==
\begin{table*}
\caption{Perfectly annotated templates for three page versions with alignment}
\label{tab:perfect_alignment}
\begin{tabular}{lrlrll}
\toprule
	&Page version			&	&Diff				&	&Annotated template \\
\midrule
v1	&Lorem 2022-04-05 ipsum 1.0 BTC	&	&		$\nearrow$	&t1	&Lorem {\color{blue}date} ipsum {\color{blue}price} BTC \\
	&		$\searrow$	&d1\_2	&Lorem {\color{red}2022-04-05}	&	& \\
	&		$\nearrow$	&	&{\color{green}2022-04-06} ipsum
							{\color{orange}1.0} BTC	&	& \\
v2	&Lorem 2022-04-06 ipsum 1.0 BTC	&	&		$\searrow$	&t2	&Lorem {\color{blue}date} ipsum {\color{blue}price} BTC \\
	&				&	&		$\nearrow$	&=t2'	&Lorem {\color{blue}date} ipsum {\color{blue}price } BTC \\
	&		$\searrow$	&d2\_3	&Lorem {\color{orange}2022-04-06}
										&	& \\
	&		$\nearrow$	&	&ipsum {\color{red}1.0} {\color{green}1.5} BTC
										&	& \\
v3	&Lorem 2022-04-06 ipsum 1.5 BTC	&	&		$\searrow$	&t3	&Lorem {\color{blue}date} ipsum {\color{blue}price} BTC \\
\bottomrule
\end{tabular}
\end{table*}


==> tables_v5/tab_summary.tex <==
\begin{table}
\caption{Diffing-as-a-lens applied to two near duplicates equal except for the date. The arrows indicate that a diff has two inputs and two outputs}
\label{tab:summary}
\begin{tabular}{lrlll}
\toprule
	&Page version		&Diff					&	&Annotated template \\
\midrule
v1	&\multicolumn{2}{l}{Lorem 2022-04-05 ipsum}	$\nearrow$	&t1	&Lorem {\color{blue}date} ipsum \\
	&	$\searrow$	&Lorem {\color{red}2022-04-05}		&	& \\
	&	$\nearrow$	&{\color{green}2022-04-06} ipsum	&	& \\
v2	&\multicolumn{2}{l}{Lorem 2022-04-06 ipsum}	$\searrow$	&t2	&Lorem {\color{blue}date} ipsum \\
\bottomrule
\end{tabular}
\end{table}

